Lie Group Algebra Convolutional Filters

In this paper we propose a framework to leverage Lie group symmetries on arbitrary spaces exploiting \textit{algebraic signal processing} (ASP). We show that traditional group convolutions are one particular instantiation of a more general Lie group algebra homomorphism associated to an algebraic signal model rooted in the Lie group algebra $L^{1}(G)$ for given Lie group $G$. Exploiting this fact, we decouple the discretization of the Lie group convolution elucidating two separate sampling instances: the filter and the signal. To discretize the filters, we exploit the exponential map that links a Lie group with its associated Lie algebra. We show that the discrete Lie group filter learned from the data determines a unique filter in $L^{1}(G)$, and we show how this uniqueness of representation is defined by the bandwidth of the filter given a spectral representation. We also derive error bounds for the approximations of the filters in $L^{1}(G)$ with respect to its learned discrete representations. The proposed framework allows the processing of signals on spaces of arbitrary dimension and where the actions of some elements of the group are not necessarily well defined. Finally, we show that multigraph convolutional signal models come as the natural discrete realization of Lie group signal processing models, and we use this connection to establish stability results for Lie group algebra filters. To evaluate numerically our results, we build neural networks with these filters and we apply them in multiple datasets, including a knot classification problem.

==> figures/1109_figures/ROT_MNIST1005.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{180, 222,44}
\definecolor{my_cp5_col3}{RGB}{94, 201, 98}
\definecolor{my_cp5_col4}{RGB}{33, 145, 140}
\definecolor{my_cp5_col5}{RGB}{59, 82, 139}
\definecolor{my_cp5_col6}{RGB}{68, 1, 84}
\definecolor{my_cp5_col7}{RGB}{49, 104, 142}
\definecolor{my_cp5_col8}{RGB}{72, 40, 120}

\definecolor{cadetblue74171164}{RGB}{74,171,164}
\definecolor{darksalmon233149163}{RGB}{233,149,163}
\definecolor{darkslategray70}{RGB}{70,70,70}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{lightsteelblue182167234}{RGB}{182,167,234}
\definecolor{mediumseagreen72175114}{RGB}{72,175,114}
\definecolor{mediumturquoise82172205}{RGB}{82,172,205}
\definecolor{peru20215175}{RGB}{202,151,75}
\definecolor{plum231140215}{RGB}{231,140,215}
\definecolor{yellowgreen15116269}{RGB}{151,162,69}
\begin{axis}[
axis background/.style={fill=gainsboro229},
axis line style={white},
tick align=outside,
tick pos=left,
title={RotMNIST},
x grid style={white},
xlabel=\textcolor{dimgray85}{Test Accuracy},
xmajorgrids,
xmin=0.318525, xmax=0.793175,
xtick style={color=dimgray85},
y dir=reverse,
y grid style={white},
ylabel=\textcolor{dimgray85}{Model},
ymin=-0.5, ymax=7.5,
ytick style={color=dimgray85},
ytick={0,1,2,3,4,5,6,7},
yticklabels={
  GrpA-1: SO(2),
  GrpA-2: SO(2),
  LieConv-1,
  LieConv-2,
  FCNN-1,
  FCNN-2,
  GrpA-1: SO(2)+,
  GrpA-2: SO(2)+
}
]
\path [draw=darkslategray70, fill=darksalmon233149163, semithick]
(axis cs:0.564935,-0.4)
--(axis cs:0.564935,0.4)
--(axis cs:0.588515,0.4)
--(axis cs:0.588515,-0.4)
--(axis cs:0.564935,-0.4)
--cycle;
\path [draw=darkslategray70, fill=peru20215175, semithick]
(axis cs:0.571395,0.6)
--(axis cs:0.571395,1.4)
--(axis cs:0.655665,1.4)
--(axis cs:0.655665,0.6)
--(axis cs:0.571395,0.6)
--cycle;
\path [draw=darkslategray70, fill=yellowgreen15116269, semithick]
(axis cs:0.65313,1.6)
--(axis cs:0.65313,2.4)
--(axis cs:0.67776,2.4)
--(axis cs:0.67776,1.6)
--(axis cs:0.65313,1.6)
--cycle;
\path [draw=darkslategray70, fill=mediumseagreen72175114, semithick]
(axis cs:0.558335,2.6)
--(axis cs:0.558335,3.4)
--(axis cs:0.685385,3.4)
--(axis cs:0.685385,2.6)
--(axis cs:0.558335,2.6)
--cycle;
\path [draw=darkslategray70, fill=cadetblue74171164, semithick]
(axis cs:0.36003,3.6)
--(axis cs:0.36003,4.4)
--(axis cs:0.46681,4.4)
--(axis cs:0.46681,3.6)
--(axis cs:0.36003,3.6)
--cycle;
\path [draw=darkslategray70, fill=mediumturquoise82172205, semithick]
(axis cs:0.49835,4.6)
--(axis cs:0.49835,5.4)
--(axis cs:0.636005,5.4)
--(axis cs:0.636005,4.6)
--(axis cs:0.49835,4.6)
--cycle;
\path [draw=darkslategray70, fill=lightsteelblue182167234, semithick]
(axis cs:0.64712,5.6)
--(axis cs:0.64712,6.4)
--(axis cs:0.70809,6.4)
--(axis cs:0.70809,5.6)
--(axis cs:0.64712,5.6)
--cycle;
\path [draw=darkslategray70, fill=plum231140215, semithick]
(axis cs:0.70958,6.6)
--(axis cs:0.70958,7.4)
--(axis cs:0.75608,7.4)
--(axis cs:0.75608,6.6)
--(axis cs:0.70958,6.6)
--cycle;
\addplot [semithick, darkslategray70]
table {%
0.564935 0
0.54652 0
};
\addplot [semithick, darkslategray70]
table {%
0.588515 0
0.5998 0
};
\addplot [semithick, darkslategray70]
table {%
0.54652 -0.2
0.54652 0.2
};
\addplot [semithick, darkslategray70]
table {%
0.5998 -0.2
0.5998 0.2
};
\addplot [semithick, darkslategray70]
table {%
0.571395 1
0.52966 1
};
\addplot [semithick, darkslategray70]
table {%
0.655665 1
0.68654 1
};
\addplot [semithick, darkslategray70]
table {%
0.52966 0.8
0.52966 1.2
};
\addplot [semithick, darkslategray70]
table {%
0.68654 0.8
0.68654 1.2
};
\addplot [semithick, darkslategray70]
table {%
0.65313 2
0.62094 2
};
\addplot [semithick, darkslategray70]
table {%
0.67776 2
0.6834 2
};
\addplot [semithick, darkslategray70]
table {%
0.62094 1.8
0.62094 2.2
};
\addplot [semithick, darkslategray70]
table {%
0.6834 1.8
0.6834 2.2
};
\addplot [semithick, darkslategray70]
table {%
0.558335 3
0.545 3
};
\addplot [semithick, darkslategray70]
table {%
0.685385 3
0.70548 3
};
\addplot [semithick, darkslategray70]
table {%
0.545 2.8
0.545 3.2
};
\addplot [semithick, darkslategray70]
table {%
0.70548 2.8
0.70548 3.2
};
\addplot [semithick, darkslategray70]
table {%
0.36003 4
0.3401 4
};
\addplot [semithick, darkslategray70]
table {%
0.46681 4
0.5087 4
};
\addplot [semithick, darkslategray70]
table {%
0.3401 3.8
0.3401 4.2
};
\addplot [semithick, darkslategray70]
table {%
0.5087 3.8
0.5087 4.2
};
\addplot [semithick, darkslategray70]
table {%
0.49835 5
0.34284 5
};
\addplot [semithick, darkslategray70]
table {%
0.636005 5
0.70664 5
};
\addplot [semithick, darkslategray70]
table {%
0.34284 4.8
0.34284 5.2
};
\addplot [semithick, darkslategray70]
table {%
0.70664 4.8
0.70664 5.2
};
\addplot [semithick, darkslategray70]
table {%
0.64712 6
0.6225 6
};
\addplot [semithick, darkslategray70]
table {%
0.70809 6
0.71542 6
};
\addplot [semithick, darkslategray70]
table {%
0.6225 5.8
0.6225 6.2
};
\addplot [semithick, darkslategray70]
table {%
0.71542 5.8
0.71542 6.2
};
\addplot [semithick, darkslategray70]
table {%
0.70958 7
0.66038 7
};
\addplot [semithick, darkslategray70]
table {%
0.75608 7
0.7716 7
};
\addplot [semithick, darkslategray70]
table {%
0.66038 6.8
0.66038 7.2
};
\addplot [semithick, darkslategray70]
table {%
0.7716 6.8
0.7716 7.2
};
\addplot [semithick, darkslategray70]
table {%
0.582 -0.4
0.582 0.4
};
\addplot [semithick, darkslategray70]
table {%
0.59851 0.6
0.59851 1.4
};
\addplot [semithick, darkslategray70]
table {%
0.66241 1.6
0.66241 2.4
};
\addplot [semithick, darkslategray70]
table {%
0.65733 2.6
0.65733 3.4
};
\addplot [semithick, darkslategray70]
table {%
0.40126 3.6
0.40126 4.4
};
\addplot [semithick, darkslategray70]
table {%
0.59502 4.6
0.59502 5.4
};
\addplot [semithick, darkslategray70]
table {%
0.70102 5.6
0.70102 6.4
};
\addplot [semithick, darkslategray70]
table {%
0.7293 6.6
0.7293 7.4
};
\end{axis}

\end{tikzpicture}


==> source_figs/fig1/fig1_tikz_source.tex <==
%!TEX root = fig1_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Blue Colors of the Palette
\definecolor{my_alejocol5a}{RGB}{1,31,75}
\definecolor{my_alejocol4a}{RGB}{3,57,108}
\definecolor{my_alejocol3a}{RGB}{0,91,150}
\definecolor{my_alejocol2a}{RGB}{100,151,177}
\definecolor{my_alejocol1a}{RGB}{179,205,224}

%--------Red Colors of the Palette
\definecolor{my_alejocol4b}{RGB}{212, 220, 220}
\definecolor{my_alejocol3b}{RGB}{113, 18, 55}
\definecolor{my_alejocol2b}{RGB}{236, 85, 141}
\definecolor{my_alejocol1b}{RGB}{225, 73, 132}

%--------Blue-Green Colors of the Palette
\definecolor{my_alejocol4c}{RGB}{81, 185, 239}
\definecolor{my_alejocol3c}{RGB}{119, 164, 211}
\definecolor{my_alejocol2c}{RGB}{193, 223, 213}
\definecolor{my_alejocol1c}{RGB}{53, 89, 85}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}



\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
%\usepackage[english]{babel}
%\usepackage{microtype}
%\usepackage[hmargin=1.5cm,vmargin=1cm]{geometry}
%\usepackage{amsmath}
%\DeclareMathOperator{\p}{p}
%\newcommand*{\cancer}{\text{cancer}}
%\newcommand*{\testp}{\text{test}+}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%

\def \scale {1.3}
\def \unit  { \scale cm}
\def \layerinterdist {2.5}


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_alejocol4c!50,
                             minimum width  = 1.5*\unit,
                             minimum height = 2.0*\unit]
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=black!15,
                              minimum height = 1.3*\unit]
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.3*\unit,
                              fill=black!30,
                              minimum width  = 0.8*\unit,
                              minimum height = 0.8*\unit
                             ]                                                                                                                                                
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_alejocol2b!70,
                        minimum width = 1.5*\unit]


\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





{\fontsize{8}{8}\selectfont


\begin{tikzpicture}[rounded corners,ultra thick]




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Vector space M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (0,0) node [vectorspace] (M0) {};
   \path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};
   
   % Element of the vector space
   \path (M0) ++ (-0.5,0.2) node [dot] (x) {};
   \path (x.south)++(0,-0.1) node [below, color=black] {$\mathbf{x}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (0.5,0.2) node [dot] (ex) {};
   \path (ex.south) node [below, color=black] {$\rho(a)\mathbf{x}$};      
              

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Endomorphisms   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   % Space of endomorphisms
   \path (M0.north) ++ (0, 0.5) 
         node [endomorphisms, anchor=south] (End0) {};
   \path (End0.north) ++ (0.0, 0) node [below, color=black] {$\text{End}(\mathcal{M})$}; 
   

   % Adding an endomorphism element 
   \path (End0.south) ++ (0.0, 0.3) node [dot] (e) {};      
   %\path (e) node [below] {$\rho_{0}(g)=\mathbf{S}_{0}$};    
   
   % Arrow going from x to Ex
   \path (e)+(-0.5,0.55) coordinate (c1);
   \path (e)+(0.5,0.55) coordinate (c2);   
   \path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x) .. controls (c1) and (c2) .. (ex);   


   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Lie Algebra (original with Bracket product)%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   % Lie Algebra    
   \path (End0.north west) ++ (-4, 0) 
         node [algebra, anchor = north east, fill=my_alejocol2b!70] (At) {};   
   \path (At.north) ++ (0,-0.1) node [below,color=black] {$\mathfrak{g}$}; 
   \path (At.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
   \path (At.south) ++ (0,-0.1) node [below,color=black] {Lie Algebra};
   \path (At.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   
%   % Subset in A_tilde  
%    \path (At.south) ++ (0,0.1) 
%    node [subendomor2in1, anchor=south,color=black!30] (subset2) {};
%    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\tilde{\mathcal{C}}$};
    
    % Element in the Algebra
    %\path (At.south) ++ (0.0, 0.2) node [dot] (a2) {}; 
   
   
   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Universal Enveloping Algebra U(g) %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (End0.north west) ++ (-1, 0) 
         node [algebra, anchor = north east] (A) {};   
   \path (A.north) ++ (0,-0.1) node [below,color=black] {$U(\mathfrak{g})$};
   \path (A.center) ++ (0,0) node [below,color=black] {$xy=z$};  
   \path (A.south) ++ (0,-0.1) node [below,color=black, align=center] {Universal\\ Enveloping \\Algebra};  
    
    
%    % Subset in the Algebra  
%    \path (A.south) ++ (0,0.1) 
%    node [subendomor2in1, anchor=south,color=black!30] (subset2) {};
%    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
    
    % Element in the Algebra
    \path (A.south) ++ (0.0, 0.2) node [dot] (a1) {}; 
        
        
        
        
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (1,-0.6) coordinate (c1);
   \path (End0.north) + (-1,-0.6) coordinate (c2);   
   \path [draw, -stealth,line width = 1.0,color=green!60!black] (a1) .. controls (c1) and (c2) .. (e) node[midway,above left,rotate=0,color=green!60!black] {$\rho$};
   
   
   
   
   % Arrow going from Lie Algebra to universal Enveloping U(g)
   \path (A.south) + (-0.2,-0.5) coordinate (c2);
   \path (At.south) + (0.2,-0.5) coordinate (c1);   
   \path [->,draw, -stealth,line width = 1,color=black] (At.east) -- (A.west) node[midway,below,rotate=0,color=black] {$U$};




\end{tikzpicture}


}







==> source_figs/fig10/fig2_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%


%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{180, 222,44}
\definecolor{my_cp5_col3}{RGB}{94, 201, 98}
\definecolor{my_cp5_col4}{RGB}{33, 145, 140}
\definecolor{my_cp5_col5}{RGB}{59, 82, 139}
\definecolor{my_cp5_col6}{RGB}{68, 1, 84}


\usetikzlibrary{positioning,decorations.pathreplacing,shapes}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SCALES AND BASIC QUANTITIES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%--- Scale 
\def \scale {1.4}
\def \unit { \scale cm}

%%--- Vertical distance between blocks
\def \vertsep {1*\scale}

%%--- Horizontal distance between blocks
\def \horzsep {1*\scale}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    SETTINGS OF BLOCKS USED IN THE PICTURE %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
 
\tikzstyle{myboxlabel} = [set,
fill=my_cp5_col3,
minimum width  = 1.61*\unit,
minimum height = 0.5*\unit]
 
 
                             

\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BEGINNING OF PICTURE %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%-- Here I can choose the font size ----
{\fontsize{8}{8}\selectfont	
	
	
\begin{tikzpicture}[scale=\scale,rounded corners,ultra thick]



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Color Labels palette  %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


   %%------------ Label 1 --------
   
   \path (0,0) node [] (L1) {};
   \path (L1) ++ (0, 0) node [rotate=90, color=black] {Label 1};
   
   
   %%------------ Label 2 --------
   
    \path (L1.south)++(0,\vertsep) node [] (L2) {};
    \path (L2) ++ (0, 0) node [rotate=90, color=black] {Label 2};
    
    
     %%------------ Label 3 --------
     
     \path (L2.south)++(0,\vertsep) node [] (L3) {};
     \path (L3) ++ (0, 0) node [rotate=90, color=black] {Label 3};  
    
    
     %%------------ Label 4 --------
         
     \path (L3.south)++(0,\vertsep) node [] (L4) {};
     \path (L4) ++ (0, 0) node [rotate=90, color=black] {Label 4}; 
    
 

\end{tikzpicture}


}







==> source_figs/fig2/fig2_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Blue Colors of the Palette
\definecolor{my_alejocol5a}{RGB}{1,31,75}
\definecolor{my_alejocol4a}{RGB}{3,57,108}
\definecolor{my_alejocol3a}{RGB}{0,91,150}
\definecolor{my_alejocol2a}{RGB}{100,151,177}
\definecolor{my_alejocol1a}{RGB}{179,205,224}

%--------Red Colors of the Palette
\definecolor{my_alejocol4b}{RGB}{212, 220, 220}
\definecolor{my_alejocol3b}{RGB}{113, 18, 55}
\definecolor{my_alejocol2b}{RGB}{236, 85, 141}
\definecolor{my_alejocol1b}{RGB}{225, 73, 132}

%--------Blue-Green Colors of the Palette
\definecolor{my_alejocol4c}{RGB}{81, 185, 239}
\definecolor{my_alejocol3c}{RGB}{119, 164, 211}
\definecolor{my_alejocol2c}{RGB}{193, 223, 213}
\definecolor{my_alejocol1c}{RGB}{53, 89, 85}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}



\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
%\usepackage[english]{babel}
%\usepackage{microtype}
%\usepackage[hmargin=1.5cm,vmargin=1cm]{geometry}
%\usepackage{amsmath}
%\DeclareMathOperator{\p}{p}
%\newcommand*{\cancer}{\text{cancer}}
%\newcommand*{\testp}{\text{test}+}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%

\def \scale {1.3}
\def \unit  { \scale cm}
\def \layerinterdist {2.5}


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
\tikzstyle{shadow_squared} = [rectangle,color=black,
rounded corners = 0.2*\unit,
fill=black,
inner sep=0pt,
draw,
anchor = south east,
line width=0.1mm,
minimum width  = 4.1*\unit,
minimum height = 3.9*\unit]                    
                    

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_alejocol4c!50,
                             minimum width  = 1.5*\unit,
                             minimum height = 2.0*\unit]
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=black!15,
                              minimum height = 1.3*\unit]
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.3*\unit,
                              fill=black!30,
                              minimum width  = 0.8*\unit,
                              minimum height = 0.8*\unit
                             ]                                                                                                                                                
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_alejocol2b!70,
                        minimum width = 1.5*\unit]

\tikzstyle{group_math} = [endomorphisms,
minimum width = 1.5*\unit,
minimum height = 0.5*\unit]


\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





{\fontsize{8}{8}\selectfont


\begin{tikzpicture}[rounded corners,ultra thick]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Shadow Under ASP Model %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 \path (0.9*\unit,-1.1*\unit) node [shadow_squared, opacity=0.2, fill=gray] (shadow1) {};
 %\path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};      






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Vector space M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (0,0) node [vectorspace] (M0) {};
   \path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};
   
   % Element of the vector space
   \path (M0) ++ (-0.5,0.2) node [dot] (x) {};
   \path (x.south)++(0,-0.1) node [below, color=black] {$\mathbf{x}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (0.5,0.2) node [dot] (ex) {};
   \path (ex.south) node [below, color=black] {$\rho(a)\mathbf{x}$};      
              

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Endomorphisms   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (M0.north) ++ (0, 0.5) 
         node [endomorphisms, anchor=south] (End0) {};
   \path (End0.north) ++ (0.0, 0) node [below, color=black] {$\text{End}(\mathcal{M})$}; 
   

   % Adding an endomorphism element 
   \path (End0.south) ++ (0.0, 0.3) node [dot] (e) {};      
   %\path (e) node [below] {$\rho_{0}(g)=\mathbf{S}_{0}$};    
   
   % Arrow going from x to Ex
   \path (e)+(-0.5,0.55) coordinate (c1);
   \path (e)+(0.5,0.55) coordinate (c2);   
   \path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x) .. controls (c1) and (c2) .. (ex);   


   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Lie Algebra (original with Bracket product)%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   % Lie Algebra    
   \path (End0.north west) ++ (-4, 0) 
         node [algebra, anchor = north east, fill=my_alejocol2b!70] (At) {};   
   \path (At.north) ++ (0,-0.1) node [below,color=black] {$\mathfrak{g}$}; 
   \path (At.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
   \path (At.south) ++ (0,-0.1) node [below,color=black] {Lie Algebra};
   \path (At.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Lie Group %%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   % Lie Group   
   \path (At.south) ++ (0, -2.5) 
   node [group_math, anchor = center, fill=my_alejocolg1!50] (G) {};   
   \path (G.north) ++ (0,-0.1) node [below,color=black] {$G$}; 
   %\path (G.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
   \path (G.south) ++ (0,-0.1) node [below,color=black] {Lie Group};
   %\path (G.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   

   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Universal Enveloping Algebra U(g) %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (End0.north west) ++ (-1, 0) 
         node [algebra, anchor = north east] (A) {};   
   \path (A.north) ++ (0,-0.1) node [below,color=black] {$U(\mathfrak{g})$};
   \path (A.center) ++ (0,0) node [below,color=black] {$xy=z$};  
   \path (A.south) ++ (0,-0.1) node [below,color=black, align=center] {Universal\\ Enveloping \\Algebra};  
    
    
%    % Subset in the Algebra  
%    \path (A.south) ++ (0,0.1) 
%    node [subendomor2in1, anchor=south,color=black!30] (subset2) {};
%    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
    
    % Element in the Algebra
    \path (A.south) ++ (0.0, 0.2) node [dot] (a1) {}; 
        
        
        
        
 
        
        
        
        
        
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (1,-0.6) coordinate (c1);
   \path (End0.north) + (-1,-0.6) coordinate (c2);   
   \path [draw, -stealth,line width = 1.0,color=green!60!black] (a1) .. controls (c1) and (c2) .. (e) node[midway,above left,rotate=0,color=green!60!black] {$\rho$};
   
   
   % Arrow going from Lie Algebra to universal Enveloping U(g)  
   \path [->,draw, -stealth,line width = 1,color=black] (At.east) -- (A.west) node[midway,below,rotate=0,color=black] {$U$};


    % Arrow going from Lie Algebra to Lie Group = Exponential Map  
    \path [->,draw, -stealth,line width = 1,color=black] (At.south)+(0,-1) -- (G.north) node[midway,right,rotate=0,color=black] {$e^{(\cdot)}$};



\end{tikzpicture}


}







==> source_figs/fig3/fig3_tikz_source.tex <==
%!TEX root = fig3_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Blue Colors of the Palette
\definecolor{my_alejocol5a}{RGB}{1,31,75}
\definecolor{my_alejocol4a}{RGB}{3,57,108}
\definecolor{my_alejocol3a}{RGB}{0,91,150}
\definecolor{my_alejocol2a}{RGB}{100,151,177}
\definecolor{my_alejocol1a}{RGB}{179,205,224}

%--------Red Colors of the Palette
\definecolor{my_alejocol4b}{RGB}{212, 220, 220}
\definecolor{my_alejocol3b}{RGB}{113, 18, 55}
\definecolor{my_alejocol2b}{RGB}{236, 85, 141}
\definecolor{my_alejocol1b}{RGB}{225, 73, 132}

%--------Blue-Green Colors of the Palette
\definecolor{my_alejocol4c}{RGB}{81, 185, 239}
\definecolor{my_alejocol3c}{RGB}{119, 164, 211}
\definecolor{my_alejocol2c}{RGB}{193, 223, 213}
\definecolor{my_alejocol1c}{RGB}{53, 89, 85}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}



\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
\usetikzlibrary{arrows}
%\usepackage[english]{babel}
%\usepackage{microtype}
%\usepackage[hmargin=1.5cm,vmargin=1cm]{geometry}
%\usepackage{amsmath}
%\DeclareMathOperator{\p}{p}
%\newcommand*{\cancer}{\text{cancer}}
%\newcommand*{\testp}{\text{test}+}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%

\def \scale {1.3}
\def \unit  { \scale cm}
\def \layerinterdist {2.5}


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
\tikzstyle{shadow_squared} = [rectangle,color=black,
rounded corners = 0.2*\unit,
fill=black,
inner sep=0pt,
draw,
anchor = south east,
line width=0.1mm,
minimum width  = 4.1*\unit,
minimum height = 3.9*\unit]                    
                    

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_alejocol4c!50,
                             minimum width  = 1.5*\unit,
                             minimum height = 2.0*\unit]
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=black!15,
                              minimum height = 1.3*\unit]
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.3*\unit,
                              fill=black!30,
                              minimum width  = 0.8*\unit,
                              minimum height = 0.8*\unit
                             ]                                                                                                                                                
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_alejocol2b!70,
                        minimum width = 1.5*\unit]

\tikzstyle{group_math} = [endomorphisms,
minimum width = 1.5*\unit,
minimum height = 0.5*\unit]


\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





{\fontsize{8}{8}\selectfont


\begin{tikzpicture}[rounded corners,ultra thick]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Shadow Under ASP Model %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 \path (0.9*\unit,-1.1*\unit) node [shadow_squared, opacity=0.2, fill=gray] (shadow1) {};
 %\path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};      

 \path (-5.9*\unit,-1.1*\unit) node [shadow_squared, opacity=0.2, fill=gray] (shadow2) {};
 %\path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};    




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Vector space M  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (0,0) node [vectorspace] (M0) {};
   \path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};
   
   % Element of the vector space
   \path (M0) ++ (-0.5,0.2) node [dot] (x) {};
   \path (x.south)++(0,-0.1) node [below, color=black] {$\mathbf{x}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (0.5,0.2) node [dot] (ex) {};
   \path (ex.south) node [below, color=black] {$\rho(a)\mathbf{x}$};      
              

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Endomorphisms   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (M0.north) ++ (0, 0.5) 
         node [endomorphisms, anchor=south] (End0) {};
   \path (End0.north) ++ (0.0, 0) node [below, color=black] {$\text{End}(\mathcal{M})$}; 
   

   % Adding an endomorphism element 
   \path (End0.south) ++ (0.0, 0.3) node [dot] (e) {};      
   %\path (e) node [below] {$\rho_{0}(g)=\mathbf{S}_{0}$};    
   
   % Arrow going from x to Ex
   \path (e)+(-0.5,0.55) coordinate (c1);
   \path (e)+(0.5,0.55) coordinate (c2);   
   \path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x) .. controls (c1) and (c2) .. (ex);   








   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Lie Algebra (original with Bracket product)%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   % Lie Algebra    
   \path (End0.north west) ++ (-4, 0) 
         node [algebra, anchor = north east, fill=my_alejocol3a] (At) {};   
   \path (At.north) ++ (0,-0.1) node [below,color=black] {\textcolor{white}{$\mathfrak{g}$}}; 
   \path (At.center) ++ (0,0) node [below,color=black] {\textcolor{white}{$[X,Y]=Z$}}; 
   \path (At.south) ++ (0,-0.1) node [below,color=black] {Lie Algebra};
   \path (At.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   
   
   
   
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%% L1(g) %%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   \path (At.north) ++ (0, 1) 
   node [algebra, anchor = south] (Lg) {};   
   \path (Lg.north) ++ (0,-0.1) node [below,color=black] {$L_1 (\mathfrak{g})$};
   \path (Lg.center) ++ (0,0) node [below,color=black] {$\tilde{f}: \mathfrak{g}\rightarrow\mathbb{C}$};  
   % \path (LUg.south) ++ (0,-0.1) node [below,color=black, align=center] {Universal\\ Enveloping \\Algebra};  
   
   
   %    % Subset in the Algebra  
   %    \path (A.south) ++ (0,0.1) 
   %    node [subendomor2in1, anchor=south,color=black!30] (subset2) {};
   %    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
   
   % Element in the Algebra
  % \path (A.south) ++ (0.0, 0.2) node [dot] (a1) {}; 
   
   
   
   
   
   
   
   
   
   
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%  L1(G) - Group Algebra %%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    % Group Algebra
    \path (At.north west) ++ (-1, 0) 
    node [algebra, anchor = north east, fill=my_alejocol2b!70] (LG) {};   
    \path (LG.north) ++ (0,-0.1) node [below,color=black] {$L_1(G)$}; 
    \path (LG.center) ++ (0,0) node [below,color=black] {$f: G\rightarrow\mathbb{C}$}; 
    \path (LG.south) ++ (0,-0.1) node [below,color=black] {Group Algebra};
    %\path (LG.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   
   
   
   
   
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%% Endomorphisms  for ASP model in L(G) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \path (LG.west) ++ (-2, 0) 
    node [endomorphisms, anchor=center] (End1) {};
    \path (End1.north) ++ (0.0, 0) node [below, color=black] {$\text{End}(\mathcal{V})$}; 
    
    
    
    
    
    
    
    
    
    % Adding an endomorphism element 
    % \path (End1.south) ++ (0.0, 0.3) node [dot] (e1) {};      
    %\path (e) node [below] {$\rho_{0}(g)=\mathbf{S}_{0}$};    
    
%    % Arrow going from x to Ex
%    \path (e)+(-0.5,0.55) coordinate (c1);
%    \path (e)+(0.5,0.55) coordinate (c2);   
%    \path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x) .. controls (c1) and (c2) .. (ex);   
    
   
   
   
   
   
   
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Vector space M for L(G) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   \path (End1.south)++(0,-0.5) node [vectorspace, anchor=north] (V) {};
   \path (V.south) ++ (0, 0) node [above, color=black] {$\mathcal{V}$};
   
%   % Element of the vector space
%   \path (V) ++ (-0.5,0.2) node [dot] (x) {};
%   \path (x.south)++(0,-0.1) node [below, color=black] {$\mathbf{x}$}; 
%   
%   % Element filtered in the vector space
%   \path (M0) ++ (0.5,0.2) node [dot] (ex) {};
%   \path (ex.south) node [below, color=black] {$\rho(a)\mathbf{x}$};      
%   
   
  
   
   
   
   
   
   
   
   
   
   
   
   
   
   
   
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%% Lie Group %%%%%%%%%%%%%%%%%%%%%%
   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   
   % Lie Group   
   \path (At.south) ++ (0, -2.5) 
   node [group_math, anchor = center, fill=my_alejocolg1!50] (G) {};   
   \path (G.north) ++ (0,-0.1) node [below,color=black] {$G$}; 
   %\path (G.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
   \path (G.south) ++ (0,-0.1) node [below,color=black] {Lie Group};
   %\path (G.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
   
   
   

   
   
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Universal Enveloping Algebra U(g) %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (End0.north west) ++ (-1, 0) 
         node [algebra, anchor = north east] (A) {};   
   \path (A.north) ++ (0,-0.1) node [below,color=black] {$U(\mathfrak{g})$};
   \path (A.center) ++ (0,0) node [below,color=black] {$xy=z$};  
   \path (A.south) ++ (0,-0.1) node [below,color=black, align=center] {Universal\\ Enveloping \\Algebra};  
    
    
%    % Subset in the Algebra  
%    \path (A.south) ++ (0,0.1) 
%    node [subendomor2in1, anchor=south,color=black!30] (subset2) {};
%    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
    
    % Element in the Algebra
    \path (A.south) ++ (0.0, 0.2) node [dot] (a1) {}; 
        
        
        
        
 
 
 
 
 
 
 
 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%% ARROWS %%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
         
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (1,-0.6) coordinate (c1);
   \path (End0.north) + (-1,-0.6) coordinate (c2);   
   \path [draw, -stealth,line width = 1.0,color=green!60!black] (a1) .. controls (c1) and (c2) .. (e) node[midway,above left,rotate=0,color=green!60!black] {$\rho$};
   
 
   % Arrow going from Lie Algebra to universal Enveloping U(g)  
   \path [->,draw, -stealth,line width = 1,color=black] (At.east) -- (A.west) node[midway,below,rotate=0,color=black] {$U$};


    % Arrow going from Lie Algebra to Lie Group = Exponential Map  
    \path [->,draw, -stealth,line width = 1,color=black] (At.south)+(0,-1) -- (G.north) node[midway,right,rotate=0,color=black] {$e^{(\cdot)}$};

    
    % Arrow going from L(G) to L(g)
    \path [->,draw, -stealth,line width = 1,color=black,<->] (LG.north) -- (Lg.west) node[midway,left,rotate=0,color=black,align=center] {Kashiwara-Vergne Theorem\\ $f\ast_G h = \tilde{f} \ast_{L_1 (\mathfrak{g})} \tilde{h}$};


    % Arrow going from G to L(G)
    \path [draw, -stealth ,line width = 1,color=black,<->] (G.west) -- (LG.east) node[midway,left,rotate=0,color=black,align=center] {};


\end{tikzpicture}


}







==> source_figs/fig6/fig3_tikz_source.tex <==
%!TEX root = fig3_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%


%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{94, 201, 98}
\definecolor{my_cp5_col3}{RGB}{33, 145, 140}
\definecolor{my_cp5_col4}{RGB}{59, 82, 139}
\definecolor{my_cp5_col5}{RGB}{68, 1, 84}



\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
\usetikzlibrary{arrows}




%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%




 


\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]




\tdplotsetmaincoords{0}{0} % view angles
\tdplotsetrotatedcoords{0}{0}{0} 



%% -- Number of elements in the grid
\def\gridnumber{6}
\def\imagesize{4}
\def\imagedotsize{5}


\def\scale{0.45}

{\fontsize{6}{6}\selectfont


\begin{tikzpicture}[scale=\scale, tdplot_rotated_coords, grid/.style={very thin,gray}]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% FIRST ROW IMAGES ON THE GRID %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%-----------------------------------------------
%%------------ ORIGINAL REGUALR GRID ---------------
%%-----------------------------------------------

%draw a grid in the x-y plane
\foreach \x in {0,1,...,\gridnumber}
\foreach \y in {0,1,...,\gridnumber}
{
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (\x,0) -- (\x,\gridnumber);
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (0,\y) -- (\gridnumber,\y);
};


% Drawing the pixels that indicate the image
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
}



%%-----------------------------------------------
%%----------- IMAGE ON REGUALR GRID ---------------
%%-----------------------------------------------

% Drawing the pixels that indicate the image
\begin{scope}[shift={(\gridnumber+1.6,-0.5)},rotate=10]
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
	\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
}
\end{scope}


% Drawing the pixels that indicate the image
\begin{scope}[shift={(\gridnumber+1,0)},rotate=0]
\foreach \x in {0,1,...,\gridnumber}
\foreach \y in {0,1,...,\gridnumber}
{
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (\x,0) -- (\x,\gridnumber);
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (0,\y) -- (\gridnumber,\y);
};
\end{scope}




%%-----------------------------------------------
%%------------ IMAGE ON REGUALR GRID --------------
%%-----------------------------------------------

% Drawing the pixels that indicate the image

\begin{scope}[shift={(2*\gridnumber+2,0)},rotate=0]
\foreach \x in {0,1,...,\gridnumber}
\foreach \y in {0,1,...,\gridnumber}
{
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (\x,0) -- (\x,\gridnumber);
	\draw[grid,rotate=0,my_cp5_col3,line width=1*\scale] (0,\y) -- (\gridnumber,\y);
};
\end{scope}


% Drawing the pixels that indicate the image
\begin{scope}[shift={(2*\gridnumber+2,0)},rotate=0]
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
	\draw[fill=my_cp5_col3, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
};
\end{scope}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SECOND ROW HOW TO DO INTERPOLATION  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%---------------------------------------------------
%%----------- IMAGE ON REGUALR DOT-GRID --------------
%%---------------------------------------------------


% Drawing the pixels that indicate the image
\begin{scope}[shift={(0,-\gridnumber-1)},rotate=0]
\foreach \x in {0,1,...,\imagedotsize}
\foreach \y in {0,1,...,\imagedotsize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=white,minimum size=15*\scale, opacity=0.5]
	(\label) at (\x+0.5,\y+0.5) {\label};
}
\end{scope}


% Drawing the pixels that indicate the image
\begin{scope}[shift={(0,-\gridnumber-1)},rotate=0]
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=my_cp5_col2,minimum size=15*\scale, opacity=0.7]
	(\label) at (\x+0.5,\y+0.5) {\label};
}
\end{scope}



%%----------------------------------------------
%%----------- IMAGE ON REGUALR GRID --------------
%%----------------------------------------------

% Drawing the pixels that indicate the image
\begin{scope}[shift={(\gridnumber+1,-\gridnumber-1)},rotate=0]
\foreach \x in {0,1,...,\imagedotsize}
\foreach \y in {0,1,...,\imagedotsize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=white,minimum size=15, opacity=0.5]
	(u\label) at (\x+0.5,\y+0.5) {\label};
}
\end{scope}


% Drawing the pixels that indicate the image
\begin{scope}[shift={(\gridnumber+1.6,-\gridnumber-1-0.5)},rotate=10]
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=my_cp5_col2,minimum size=15, opacity=0.7]
	(v\label) at (\x+0.5,\y+0.5) {\label};
}
\end{scope}


%%---------- Neightborhood for interpolation ------------------

\node[circle,fill=my_cp5_col4,draw,opacity=0.4,inner sep=20pt] () at (u7){};


\node[dot,draw=black,fill=my_cp5_col3,minimum size=15, opacity=0.7](u7) at (u7) {7};


%%----------------------------------------------
%%----------- IMAGE ON REGUALR GRID --------------
%%----------------------------------------------

% Drawing the pixels that indicate the image
\begin{scope}[shift={(2*\gridnumber+2,-\gridnumber-1)},rotate=0]
\foreach \x in {0,1,...,\imagedotsize}
\foreach \y in {0,1,...,\imagedotsize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=white,minimum size=15, opacity=0.5]
	() at (\x+0.5,\y+0.5) {\label};
}
\end{scope}


% Drawing the pixels that indicate the image
\begin{scope}[shift={(2*\gridnumber+2,-\gridnumber-1)},rotate=0]
\foreach \x in {1,...,\imagesize}
\foreach \y in {1,...,\imagesize}
{
	%\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
	%\node[circle,draw=black,fill=white!80!black,minimum size=20] () at (\x+0.5,\y+0.5) {d};
	\pgfmathtruncatemacro{\label}{\x + 5 * (4 - \y)+6};
	\node[dot,draw=black,fill=my_cp5_col3,minimum size=15, opacity=0.7]
	() at (\x+0.5,\y+0.5) {\label};
}
\end{scope}





%% Drawing the pixels that indicate the image
%\begin{scope}[shift={(\gridnumber+1.6,-0.5)},rotate=10]
%
%
%\foreach \x in {1,...,\imagesize}
%\foreach \y in {1,...,\imagesize}
%{
%	\draw[fill=my_cp5_col2, opacity=0.7]  (\x,\y,0) -- (\x+1,\y,0) -- (\x+1,\y+1,0) -- (\x,\y+1,0) -- cycle;
%}
%
%\end{scope}
%
%
%% Drawing the pixels that indicate the image
%\begin{scope}[shift={(\gridnumber+1,0)},rotate=0]
%
%\foreach \x in {0,1,...,\gridnumber}
%\foreach \y in {0,1,...,\gridnumber}
%{
%	\draw[grid,rotate=0,my_cp5_col3,line width=1] (\x,0) -- (\x,\gridnumber);
%	\draw[grid,rotate=0,my_cp5_col3,line width=1] (0,\y) -- (\gridnumber,\y);
%};
%
%\end{scope}



\end{tikzpicture}   


}







==> source_figs/fig7/fig2_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%-- Four colors Color Palette
\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
\definecolor{my_cp4_col4}{RGB}{99, 143, 169}

%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{94, 201, 98}
\definecolor{my_cp5_col3}{RGB}{33, 145, 140}
\definecolor{my_cp5_col4}{RGB}{59, 82, 139}
\definecolor{my_cp5_col5}{RGB}{68, 1, 84}





\usetikzlibrary{positioning,decorations.pathreplacing,shapes}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SCALES AND BASIC QUANTITIES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%--- Scale 
\def \scale {1.4}
\def \unit { \scale cm}

%%--- Vertical distance between blocks
\def \vertsep {0.5*\scale}

%%--- Horizontal distance between blocks
\def \horzsep {0.5*\scale}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    SETTINGS OF BLOCKS USED IN THE PICTURE %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
\tikzstyle{shadow_squared} = [rectangle,color=black,
rounded corners = 0.2*\unit,
fill=black,
inner sep=0pt,
draw,
anchor = south east,
line width=0.1mm,
minimum width  = 4.1*\unit,
minimum height = 3.9*\unit]                    
                    

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_cp5_col4,
                             minimum width  = 1.61*\unit,
                             minimum height = 1*\unit]
 
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=my_cp5_col3,
                              minimum width  = 1.61*\unit,
                              minimum height = 1*\unit]
                                
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.2*\unit,
                              fill=black!30,
                              minimum width  = 1.2*\unit,
                              minimum height = 0.5*\unit
                             ]    
                             
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in2} = [endomorphisms, rounded corners=0.2*\unit,
fill=black!30,
minimum width  = 0.5*\unit,
minimum height = 0.5*\unit
]                                
 
                                                                                                                                                                         
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_cp5_col2]


\tikzstyle{group_math} = [endomorphisms]



\tikzstyle{liea_bracket} = [endomorphisms]



\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BEGINNING OF PICTURE %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%-- Here I can choose the font size ----
{\fontsize{8}{8}\selectfont	
	
	
\begin{tikzpicture}[scale=\scale,rounded corners,ultra thick]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Shadow Under ASP Model %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 %\path (0.9*\unit,-1.1*\unit) node [shadow_squared, opacity=0.2, fill=gray] (shadow1) {};
 %\path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};      






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Vector space M  %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (0,0) node [vectorspace,fill=my_cp5_col5] (M0) {};
   \path (M0.south) ++ (0, 0) node [below, color=black] {$\mathcal{H}$};
   
   % Element of the vector space
   \path (M0) ++ (-0.5,0.2) node [dot,color=white] (x) {};
   \path (x.south)++(0,-0.1) node [below, color=white] {$\mathbf{x}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (0.5,0.2) node [dot,color=white] (ex) {};
   \path (ex.south) node [below, color=white] {$\widehat{p_{\epsilon}(\mathcal{S})}\mathbf{x}$};      
     
              



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Endomorphisms   %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (M0.north) ++ (0, \vertsep) node [endomorphisms, anchor=south,fill=my_cp5_col4] (End0) {};
   \path (End0.north) ++ (0.0, 0) node [above, color=black] {$\mathcal{B}(\mathcal{H})$}; 

  %%----------------------
  %%---- Image of approximated Group Algebra
  
  \path (End0.south) ++ (0, 0.1) 
  node [ subendomor2in1, anchor = south, fill=my_cp5_col4!50] (Endhat) {};  
  \path (Endhat.north) ++ (0,-0.05) node [above,color=white] {$\rho( L^{1}(\widehat{G}))$};    

  %%----------------------
  %%---- Adding elements inside the boxes

   % Adding an endomorphism element 
   \path (End0.center) ++ (-0.5, 0.2) node [dot] (e) {};      
   \path (e) node [above,color=white] {$\rho(\boldsymbol{a})$};    
   
   % Adding an endomorphism element 
   \path (Endhat.south) ++ (0.0, 0.1) node [dot] (eepsilon) {};      
   \path (eepsilon) node [above] {$\widehat{p_{\epsilon}(\mathcal{S})}$};  
   
   % Arrow going from x to Ex
   \path (eepsilon)+(-0.5,0.4) coordinate (c1);
   \path (eepsilon)+(0.5,0.4) coordinate (c2);   
   \path [draw, -stealth, line width=0.5,color=my_cp5_col3] (x) .. controls (c1) and (c2) .. (ex);   

  

  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Algebra %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   \path (End0.north west) ++ (-\horzsep, 0) 
         node [algebra, anchor = north east,fill=my_cp5_col3] (A) {};   
   \path (A.north) ++ (0,0.0) node [above,color=black] {$\mathcal{A} = L^{1}(G)$};
   %\path (A.center) ++ (0,0) node [below,color=black] {$xy=z$};  
   % \path (A.south) ++ (0,-0.1) node [below,color=black, align=center] {Lie Group \\ Algebra};  

  %%----------------------
  %%---- Approximated Group Algebra
  %%----------------------  
  
  \path (A.south) ++ (0, 0.1) 
  node [ subendomor2in1, anchor = south, fill=my_cp5_col3!50] (LGhat) {};    
  \path (LGhat.north) ++ (0,-0.05) node [above,color=black] {$ L^{1}(\widehat{G})$};  
    
    % Element in the Algebra
    \path (LGhat.south) ++ (0.0, 0.1) node [dot] (pepsilon) {}; 
   \path (pepsilon.north) ++ (0,0.0) node [above,color=black] {$p_{\epsilon}(\widehat{\mathcal{G}})$};    
        
    % Element in the Algebra L1(G)
    \path (A.center) ++ (0.5, 0.2) node [dot] (a1) {}; 
    \path (a1.north) ++ (0,0.0) node [above,color=black] {$\boldsymbol{a}$};   
   
   
   
        
   
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%% Lie Group %%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
  % Lie Group   
  \path (A.north west) ++ (-\horzsep, 0) 
  node [group_math, anchor = north east, fill=my_cp5_col2] (G) {};   
  \path (G.north) ++ (0,0) node [above,color=black] {$G$}; 
  %\path (G.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
 % \path (G.south) ++ (0,-0.1) node [below,color=black] {Lie Group};
  %\path (G.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
    
 %%----------------------
 %%---- Approximated Group from discretization of t in exp(tX) 
 %%----------------------  
 
 \path (G.south) ++ (0, 0.1) 
  node [ subendomor2in1, anchor = south, fill=my_cp5_col2!50] (Ghat) {}; 
  \path (Ghat.north) ++ (0,0.0) node [above,color=black] {$\widehat{G}$};  

  %%----------------------
  %%---- Subset of generators in the approximated Lie Group
  %%----------------------  
  
  \path (Ghat.center) ++ (0, 0) 
  node [ subendomor2in2, anchor = center, fill=my_cp5_col2!30] (Ghatgen) {}; 
  \path (Ghatgen) ++ (0,0.0) node [color=black] {$\widehat{\mathcal{G}}$};     
        
 
 
 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%% Lie Algebra Bracket  %%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
  % Lie Algebra Bracket  
  \path (G.south) ++ (0, -\vertsep) 
  node [liea_bracket, anchor = north, fill=my_cp5_col1] (gbracket) {};   
  \path (gbracket.south) ++ (0,0) node [below,color=black] {$(\mathfrak{g},[\cdot,\cdot])$}; 
  %\path (G.center) ++ (0,0) node [below,color=black] {$[X,Y]=Z$}; 
 % \path (G.south) ++ (0,-0.1) node [below,color=black] {Lie Group};
  %\path (G.south) ++ (0,-0.5) node [below,color=black] {$X,Y,Z \in\mathfrak{g}$};
     
  %%----------------------
  %%---- Subset of generators in the LieBracket Algebra
  %%----------------------  
  
  \path (gbracket.center) ++ (0, 0) 
  node [ subendomor2in2, anchor = center, fill=my_cp5_col1!50] (gbracketgen) {}; 
  \path (gbracketgen) ++ (0,0.0) node [color=black] {$\mathfrak{G}$};  
 
 
 
 
 
 
        
        
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%% ARROWS %%%%%%%%%%%%%%%%%%%%%%      
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
  

%    % Arrow going from Lie Algebra to Lie Group = Exponential Map 
%    \path (A.west) ++ (0.15, 0) node [] (a1) {};  
%    \path [->,draw, -stealth,line width = 0.5,color=black] (G.east) -- (a1) node[midway,right,rotate=0,color=black] {};

  
     % Arrow indicating \rho going from A to End(M)  
     \path (A.north) + (1,0) coordinate (c1);
     \path (End0.north) + (-1,0) coordinate (c2);   
     \path [draw, -stealth,line width = 0.5,color=black] (a1) .. controls (c1) and (c2) .. (e)  node[midway,above ,rotate=0,color=black] {$\rho$};
        
        
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (1,-0.5) coordinate (c1);
   \path (End0.north) + (-1,-0.5) coordinate (c2);   
   \path [draw, -stealth,line width = 0.5,color=black] (pepsilon) .. controls (c1) and (c2) .. (eepsilon) node[midway,below left,rotate=0,color=black] {$\hat{\rho}$};
   

    % Arrow going from Lie Group to Lie Group Algebra
   %\path (A.south) ++ (0.0, -0.6) node [] (a1) {};  
   \path [->,draw, -stealth,line width = 0.5,color=black] (G.east) -- (A.west) node[midway,right,rotate=0,color=black] {};


    % Exponential Map grom the Lie bracket algebra into the Lie group G
    \path [->,draw, -stealth,line width = 0.5,color=black] (gbracket.north) -- (G.south) node[midway,right,rotate=0,color=black] {$e^{\mathfrak{g}t}$};


     % Exponential Map grom the Lie bracket algebra into the Lie group G
     \node (a) at (gbracket.center) {};
     \node (b) at (Ghat.center) {};
     \path [->, draw, -stealth,line width = 0.5,color=black] (a) edge [bend left]  node[midway,left,rotate=0,color=black] {$e^{\mathfrak{G}n\epsilon}$} (b);


\end{tikzpicture}


}







==> source_figs/fig8/fig2_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%-- Four colors Color Palette
\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
\definecolor{my_cp4_col4}{RGB}{99, 143, 169}

%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{94, 201, 98}
\definecolor{my_cp5_col3}{RGB}{33, 145, 140}
\definecolor{my_cp5_col4}{RGB}{59, 82, 139}
\definecolor{my_cp5_col5}{RGB}{68, 1, 84}





\usetikzlibrary{positioning,decorations.pathreplacing,shapes}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SCALES AND BASIC QUANTITIES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%--- Scale 
\def \scale {1.4}
\def \unit { \scale cm}

%%--- Vertical distance between blocks
\def \vertsep {0.5*\scale}

%%--- Horizontal distance between blocks
\def \horzsep {0.5*\scale}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    SETTINGS OF BLOCKS USED IN THE PICTURE %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
\tikzstyle{shadow_squared} = [rectangle,color=black,
rounded corners = 0.2*\unit,
fill=black,
inner sep=0pt,
draw,
anchor = south east,
line width=0.1mm,
minimum width  = 4.1*\unit,
minimum height = 3.9*\unit]                    
                    

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_cp5_col4,
                             minimum width  = 1.61*\unit,
                             minimum height = 1*\unit]
 
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=my_cp5_col3,
                              minimum width  = 1.61*\unit,
                              minimum height = 1*\unit]
                                
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.2*\unit,
                              fill=black!30,
                              minimum width  = 1.2*\unit,
                              minimum height = 0.5*\unit
                             ]    
                             
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in2} = [endomorphisms, rounded corners=0.2*\unit,
fill=black!30,
minimum width  = 0.5*\unit,
minimum height = 0.5*\unit
]                                
 
                                                                                                                                                                         
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_cp5_col2]


\tikzstyle{group_math} = [endomorphisms]



\tikzstyle{liea_bracket} = [endomorphisms]



\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BEGINNING OF PICTURE %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%-- Here I can choose the font size ----
{\fontsize{7}{7}\selectfont	
	
	

\begin{tikzpicture}[every tree node/.style={},
level distance=1.25cm,sibling distance=1mm, 
edge from parent path={(\tikzparentnode) -- (\tikzchildnode)}]



\Tree [.\node[fill=my_cp5_col2] {$\mathbf{I}$}; 
%%
%%------ Descending from S1 ------
%%
[.\node[fill=my_cp5_col3] {$\mathbf{S}_1$};  
%\edge node[auto=right] {Help!};  
              [.\node[fill=my_cp5_col4,text=my_cp5_col1]{$\mathbf{S}_{1}^{2}$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
              [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_1 \mathbf{S}_2 $}; {$\cdots$} {$\cdots$} {$\cdots$}   ] 
              [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_1 \mathbf{S}_3 $}; {$\cdots$} {$\cdots$} {$\cdots$}   ] 
]
%%
%%------ Descending from S2 ------
%%
[.\node[fill=my_cp5_col3] {$\mathbf{S}_2$}; 
              [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{2} \mathbf{S}_1$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
              [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{2}^2$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
              [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{2}\mathbf{S}_{3}$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
] 
%%
%%------ Descending from S3 ------
%%
[.\node[fill=my_cp5_col3] {$\mathbf{S}_3$}; 
             [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{3} \mathbf{S}_1$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
             [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{3}\mathbf{S}_{2}$};  {$\cdots$} {$\cdots$} {$\cdots$}  ] 
             [.\node[fill=my_cp5_col4,text=my_cp5_col1] {$\mathbf{S}_{3}^2$}; {$\cdots$} {$\cdots$} {$\cdots$}  ] 
] 
]
\end{tikzpicture}
}







==> source_figs/fig9/fig2_tikz_source.tex <==
%!TEX root = fig2_standalone.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%


%-- Viridis Color Palette
\definecolor{my_cp5_col1}{RGB}{253, 231, 37}
\definecolor{my_cp5_col2}{RGB}{180, 222,44}
\definecolor{my_cp5_col3}{RGB}{94, 201, 98}
\definecolor{my_cp5_col4}{RGB}{33, 145, 140}
\definecolor{my_cp5_col5}{RGB}{59, 82, 139}
\definecolor{my_cp5_col6}{RGB}{68, 1, 84}


\usetikzlibrary{positioning,decorations.pathreplacing,shapes}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SCALES AND BASIC QUANTITIES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%--- Scale 
\def \scale {1.4}
\def \unit { \scale cm}

%%--- Vertical distance between blocks
\def \vertsep {0.5*\scale}

%%--- Horizontal distance between blocks
\def \horzsep {1*\scale}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%    SETTINGS OF BLOCKS USED IN THE PICTURE %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]
                    
% Block styles
 
\tikzstyle{myboxlabel} = [set,
fill=my_cp5_col3,
minimum width  = 1.61*\unit,
minimum height = 0.5*\unit]
 
 
                             

\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% BEGINNING OF PICTURE %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%-- Here I can choose the font size ----
{\fontsize{8}{8}\selectfont	
	
	
\begin{tikzpicture}[scale=\scale,rounded corners,ultra thick]



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Color Labels palette  %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


   %%------------ Label 1 --------
   
   \path (0,0) node [myboxlabel,fill=my_cp5_col1] (L1) {};
   \path (L1.south) ++ (0, 0) node [below, color=black] {Label 1};
   
   
   %%------------ Label 2 --------
   
    \path (L1.east)++(\horzsep,0) node [myboxlabel,fill=my_cp5_col2] (L2) {};
    \path (L2.south) ++ (0, 0) node [below, color=black] {Label 1};
    
    
     %%------------ Label 3 --------
     
     \path (L2.east)++(\horzsep,0) node [myboxlabel,fill=my_cp5_col3] (L3) {};
     \path (L3.south) ++ (0, 0) node [below, color=black] {Label 1};  
    
    
     %%------------ Label 4 --------
         
     \path (L3.east)++(\horzsep,0) node [myboxlabel,fill=my_cp5_col4] (L4) {};
     \path (L4.south) ++ (0, 0) node [below, color=black] {Label 1}; 
    
 
      %%------------ Label 5 --------
      
      \path (L4.east)++(\horzsep,0) node [myboxlabel,fill=my_cp5_col5] (L5) {};
      \path (L5.south) ++ (0, 0) node [below, color=black] {Label 1};    
    

      %%------------ Label 6 --------
      
      \path (L5.east)++(\horzsep,0) node [myboxlabel,fill=my_cp5_col6] (L6) {};
      \path (L6.south) ++ (0, 0) node [below, color=black] {Label 1};      
    
    
    
%   % Element of the vector space
%   \path (M0) ++ (-0.5,0.2) node [dot,color=white] (x) {};
%   \path (x.south)++(0,-0.1) node [below, color=white] {$\mathbf{x}$}; 
%   
%   % Element filtered in the vector space
%   \path (M0) ++ (0.5,0.2) node [dot,color=white] (ex) {};
%   \path (ex.south) node [below, color=white] {$\widehat{p_{\epsilon}(\mathcal{S})}\mathbf{x}$};      
%     



\end{tikzpicture}


}







==> v24/LieSP.tex <==
\section{Lie Convolutions with Sampled Data}
Let $\ccalM_\ccalS:= \left\{s_i \in \ccalM\right\}$ for $i = 1, \dots, n$ be a sampling of the vector space and $\theta_\ccalS: \ccalX \to \ccalX_\ccalS$ be the projection of the continuous signal to the sampled space $\ccalX_\ccalS:\ccalM_\ccalS \to \mbR$. In the case of images, for example, $\ccalM_\ccalS$ represents the set of pixels. Using the sampled signals, we let $\left(\ccalA, \ccalM_\ccalS, \rho_\ccalS\right)$ be the sampled ASP model where $\rho_\ccalS:\ccalA \to \End{\ccalM_\ccalS}$.

%
%In practice, the continuous signal $\ccalX$ is measured by a sampling $\ccalS$. Let $\ccalX_\ccalS$ be the sampling of the continuous signal on a finite number of points $\ccalS := \left\{s_i \in \ccalX\right\}$ for $i = 1, \dots, n$. Further, let $\theta_\ccalS: \ccalX \to \ccalX_\ccalS$ be an operator which maps the continuous signal to the sampled signal. Given that $\rho(a)$ is a continuous filter, it no longer holds that $\bby$ from \eqref{equ:input_output} is an element of $\ccalX_\ccalS$. Instead, given the sampling $\ccalS$, we define the sampled ASP model to be $\left(\ccalA, \ccalM_\ccalS, \rho_\ccalS\right)$. 
This admits the input-output relation
\begin{equation} \label{equ:input_output_sampled}
    \bby_\ccalS = \rho(a)_\ccalS \theta_\ccalS(\bbx),
\end{equation}
where the subscript $\ccalS$ shows the sampling of the continuous signal. Ideally, one would want to able to obtain the homomorphism $\rho_\ccalS$ such that the sampling of \eqref{equ:input_output} is equivalent to the output of \eqref{equ:input_output_sampled}. Namely, we want $\theta_\ccalS(\bby)$ to be equivalent to $\bby_\ccalS$. As such, we aim to approximate the homomorphism $\hat \rho$ which minimize this difference. That is, 
\begin{equation}
    \hat \rho := \arg \min_{\rho_\ccalS} \left\| \rho_\ccalS(a)\theta_\ccalS(\bbx) - \theta_\ccalS(\rho(a)\bbx)\right\|.
\end{equation}
In section \ref{sec:bary_interp}, we show that this problem is well studied.



==> v24/barycentric_interpolation.tex <==
\section{Homomorphism Approximation via Interpolation} \label{sec:bary_interp}

In this section, we will describe the process of constructing the approximation of the shift operators (or discrete group actions) on the discretized vector space. In particular, let $\ccalM_\ccalS$ be the sampled vector space on which we have the signal $\ccalX:\ccalM_\ccalS\to \mbR$. Let $T(g)$ be a transformation which acts on the elements of the continuous vector space $\ccalM$. For brevity in notation, we allow $T$ to represent $T(g)$ for any group element $g\in \ccalG$.

Any element in $\ccalX$ can be represented by $\left\{\left(s_i, f(s_i)\right)\right\}_{i = 0}^{n-1}$, where $s_i \in \ccalM_\ccalS$, and $f(s_i) \in \mbR$. The continuous transformation $T$ acting on $s_i$ is an element of the continuous vector space $\ccalM$. That is, $Ts_i\in \ccalM$ for all $i = 0, \dots, n-1$. As described in Section \ref{sec:derivation}, we want to find $\hat T$ such that $\hat Ts_i\in \ccalM_\ccalS$ and \eqref{equ:sampling_problem} holds. 

Unsurprisingly, we solve the problem of finding the transformation approximation $\hat T$ with interpolation. In particular, for each $s_i$, we find the $k$-nearest neighbors (note that we use Euclidean norm due to working on Lie Groups) of $Ts_i$ in the original $\left\{s_i\right\}_{i = 0}^{n-1}$ as well as their distances. We let $\textrm{KNN}(i)$ be the set of neighbors of $Ts_i$. Then, each $Ts_i$ will have $k$ neighbors,  $s_{\textrm{KNN}(i)}$ with corresponding distances $d_{\textrm{KNN}(i)}$. The weight assigned to each neighbor, $w_{\textrm{KNN}(i)}$ should be inversely proportional to the distances. The approximation $\hat T$ should be constructed by populating an $n\times n$ matrix by the weights in the corresponding locations. 

\begin{equation}
\left[
  \begin{array}{ccc}
    \dots & \dots & \dots \\
    \dots & \dots & \dots \\
    \rule[.5ex]{2.5ex}{0.5pt} & w(i)^T & \rule[.5ex]{2.5ex}{0.5pt} \\
    \dots & \dots & \dots \\  
  \end{array}
\right]
\begin{bmatrix}
           f(s_0) \\
           f(s_1) \\
           \vdots \\
           f(s_{n-1})
         \end{bmatrix}
= 
\begin{bmatrix}
          \vdots \\
           \vdots \\
           \sum_{\textrm{KNN}(i)} w_i f(s_i) \\
           \vdots
         \end{bmatrix}.
\end{equation}

The matrix $\hat T$ is computed offline, and depends on the geometry of the problem. Additionally, when $k \ll n$, $\hat T$ is sparse having only $k^2/n^2$ of its elements filled. 

The choice of weighting is completely up to the designer. 

==> v24/lie_group_convolutions.tex <==
%!TEX root =../compiler_paper.tex






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Lie Group Convolutions}

%\blue{In this section, we will describe what is generally done to compute the lie group convolution. Namely, a signal must be lifted from the vector space to define the group measure. At that point, the convolution is performed by a discretization on the Haar measure. }

%\red{Harshat: Perhaps it's better to present the problem as an Algebraic Signal Processing model on the Group Algebra directly? For example...}

Consider the continuous vector space $\ccalM$ on top of which we define a signal $\ccalX:\ccalM \to \mbR$. Let $\ccalL$ be a Lie group, or a smooth manifold that is a group, that describes the symmetry of the signal $\ccalX$. Given the Lie Group $\ccalL$, for a field $\mbK$, we define the group algebra $\ccalA = \left\{\sum_\ccalL h(g)g\right\}$ where $h:\ccalL \to \mbK$. By construction, $\ccalA$ is unital and associative. As such, we can consider the Algebraic Signal Processing (ASP) model $\left(\ccalA, \ccalM, \rho\right)$, where $\ccalA$ is the group algebra, $\ccalM$ is a vector space, and $\rho:\ccalA \to \End{\ccalM}$ is a homomorphism between $\ccalA$ and the the set of endomorphisms in $\ccalM$ . 


In an ASP model, the filters are elements of the algebra and the signals are elements of the vector space. By applying the homomorphism on the abstract filter $a\in \ccalA$, we recover a concrete filter which acts on the signal $\bbx \in \ccalX$ to produce the input-output relation
\begin{equation} \label{equ:input_output}
    \bby = \rho(a)\bbx,
\end{equation}
where, by $\rho(a)\in \End{\ccalM}$, it follows that $\bby \in \ccalX$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%       S U B S E C T I O N             %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Algebraic Filtering}
As shown in \cite{puschel2008algebraic,parada2021algebraic, parada2021convolutional}, algebraic filters can be constructed by considering polynomials on the generators of the algebra. We review the relevant definitions and consequences in this section, particularized to the Lie Group Algebras discussed in the previous section. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%       D E F I N I T I O N             %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}\label{def:generators}\emph{(Generators)}   The set $\ccalG \in \ccalA$ generates $\ccalA$ if all $a \in \ccalA$ can be represented as polynomial functions of the elements of $\ccalG$. We say elements $g \in \ccalG$ generators of $\ccalA$, and we denote by $a = P_{\ccalA}(\ccalG)$ the polynomial that generates $a$.
\end{definition}

The representation of the generator $\rho(g)$ plays a central role in ASP. These are formally defined as shift operators, which we define next. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%       D E F I N I T I O N             %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{definition}\label{def:shift_operators}\emph{(Shift Operators)} Let $\left(\ccalA, \ccalM, \rho\right)$ be an algebraic signal processing model. Further, let $\ccalG \subset \ccalA$ be the generators of $\ccalA$ (c.f. Definition \ref{def:generators}). The shift operators are defined as the representation of the generators \begin{equation}
    \mathbf{L} = \rho(g), ~\textrm{for all}~g\in \ccalG.
\end{equation}
\end{definition}

From Definition \ref{def:shift_operators}, it follows that the image of $\rho$ can be written as a polynomial on the shift operators. To be more precise, the filter $\rho(a)$ can be generated by 
\begin{equation}
    \rho(a) = \rho\left(P_{\ccalA}(\ccalG)\right) = P_\ccalM \left(\rho(\ccalG)\right) = P_\ccalM(\textbf{L}).
\end{equation}





==> v24/sec_conventional_group_convolutions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% SUBSECTION %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Comparison to Conventional Group Signal Processing}
\label{sec_cgsp}

In group signal processing, signals and filters of interest are functions defined \textit{on} the group, and the notion of convolution leverages integration with a Haar measure~\cite{folland2016course,deitmar2014principles,hewitt1994abstract}. We recall that a left Haar measure on a group $G$ is a nonzero Radon measure $\mu$ on $G$ such that $\mu(xE)=\mu(E)$ for any Borel set $E\subset G$ and any group element $x\in B$. As pointed out in~\cite{folland2016course} (Theorem~2.10) every locally compact group has a left Haar measure. Let us denote by $C_{c}(G)$ the set of compactly supported continuous functions on $G$ and $L_{y}\boldsymbol{f}(x) = \boldsymbol{f}(y^{-1}x)$ for $\boldsymbol{f}\in C_{c}(G)$. If $\mu$ is a left Haar measure, then for any $\boldsymbol{f}\in C_{c}(G)$ it follows that

%
%
%
\begin{equation}
 \int_G   L_{y}\boldsymbol{f} d\mu 
 =
 \int_G \boldsymbol{f} d\mu
 .
\end{equation}
%
%
%

As indicated in~\cite{folland2016course} for any Lie group it is possible to derive a Haar measure using tools from differential and Riemmanian geometry -- see Appendix XXX for examples of Haar measures. 

Working on a space of measures, the Haar measure itself allows the definition of a convolution measure~\cite{folland2016course}, which can be formulated considering functions on $L^{1}(G)$ which is given by

%
%
%
\begin{equation}
 L^1 (G)
       =
       \left\lbrace 
               \boldsymbol{f}\in C_{c}(G) 
       \left\vert
                \int_G \vert \boldsymbol{f}\vert d\mu
                <\infty
       \right.            
       \right\rbrace
       .
\end{equation}
%
%
%

Then, for any  $\boldsymbol{f},\boldsymbol{g} \in L^{1}(G)$ we define the convolution according to

%
%
%
\begin{equation}\label{eq_conv_LieG_classic}
\left(
      \boldsymbol{f} \ast \boldsymbol{g}
\right)(x)
=
 \int_G \boldsymbol{f}(y)\boldsymbol{g}\left( y^{-1}x \right) d\mu(y)
 .
\end{equation}
%
%
%

Then, convolutional filtering of information living on a Lie group is computed via~\eqref{eq_conv_LieG_classic}. In particular, one could consider that in~\eqref{eq_conv_LieG_classic} $\boldsymbol{f}$ is a signal and $\boldsymbol{g}$ is a filter. Notice that the notion of group signal processing on discrete groups as presented in~\cite{terrasFG, steinbergrepg} and given according to
%
%
%
\begin{equation}
\left( 
      \boldsymbol{f}
      \ast
      \boldsymbol{g}
\right)(x)
      =
      \sum_{y\in G}
      \boldsymbol{f}(y)
      \boldsymbol{g}\left( y^{-1}x\right)
      ,
\end{equation}
%
%
%
is a particular case of~\eqref{eq_conv_LieG_classic}. This can be seen when selecting the Haar measure as $\mu (H) = \vert H\vert/\vert G\vert$, where $H\subset G$ and $\vert H \vert$ and $\vert G\vert$ indicate the number of elements in $H$ and $G$, respectively~\cite{hewitt1994abstract}(page 198).


It is important to emphasize that, it is possible to formulate a notion of convolution considering the operator $R_{y}\boldsymbol{f}(x) = \boldsymbol{f}(xy)$ instead of $L_{y}\boldsymbol{f}(x) = \boldsymbol{f}(y^{-1}x)$. Additionally, the derived convolutions can be related using the modular function of the group. We recall that if $\mu$ is a left Haar measure on the group $G$ and $x\in G$ we can define another measure $\mu_{x}(E) = \mu (Ex)$. As shown in~\cite{folland2016course} there exists a unique function $\Delta (x)$ -- independent of $\mu$ -- such that $\mu_{x} = \Delta(x)\mu$. The term $\Delta: G \rightarrow (0,\infty)$ is known as the modular function of $G$. As shown in~\cite{folland2016course} we have that

%
%
%
\begin{equation}
\int_G R_{y}\boldsymbol{f}d\lambda 
       = 
       \Delta(y^{-1})\int_G \boldsymbol{f}d\mu
.
\end{equation}
%
%
%
Additionally, it can be shown that if $z\in G$ is a fixed element we have $d\lambda (xz) = \Delta(z)d\lambda (x)$. When $\Delta (x) = 1$ for all $x\in G$ we say that $G$ is unimodular. In this scenario we have that left and right Haar measures are equal. As pointed out in~\cite{hewitt1994abstract,folland2016course} discrete groups, finite groups, compact groups, connected semi-simple Lie groups, and nilpotent connected Lie groups are all unimodular, i.e $\Delta(x)=1$ for all $x\in G$. It is important to remark that the \textit{invariance} to the actions of $L_{y}$ and $R_{y}$ used in the convolutions is given by $L_{y}(\boldsymbol{f}\ast\boldsymbol{g}) = (L_{y}\boldsymbol{f})\ast \boldsymbol{g}$ and $R_{y}(\boldsymbol{f}\ast\boldsymbol{g}) = \boldsymbol{f}\ast ( R_{y}\boldsymbol{g})$.


==> v24/sec_extra_temporal_file.tex <==
%!TEX root =../compiler_paper.tex






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of ***}

\begin{multline}
\left\Vert 
    \rho(\boldsymbol{a})
    -
    \widehat{
    \rho\left(
             \boldsymbol{p}_{\boldsymbol{a}, \epsilon}
         \right)
             }
\right\Vert
=
\left\Vert 
    \rho(\boldsymbol{a})
    -
    \rho\left( 
          \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                 \left(
                      \widehat{\ccalG}
                 \right)
         \right)
    -
    \boldsymbol{\xi} \{  \boldsymbol{p}_{\boldsymbol{a},\epsilon} \}
\right\Vert
\end{multline}

Now, xxxxxxxxxxxxxxxxxxxxxxx

\begin{multline}
\left\Vert 
    \rho(\boldsymbol{a})
    -
    \rho\left( 
          \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                 \left(
                      \widehat{\ccalG}
                 \right)
         \right)
    -
    \boldsymbol{\xi} \{  \boldsymbol{p}_{\boldsymbol{a},\epsilon} \}
\right\Vert
=
\\
\left\Vert 
   \rho(\boldsymbol{a})
    -
    \rho\left( 
          \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                 \left(
                      \widehat{\ccalG}
                 \right)
         \right)
    -
    \boldsymbol{\xi} \{  \boldsymbol{p}_{\boldsymbol{a},\epsilon} \}
    +
    \rho\left( 
             \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                     \{ \ccalG \}
        \right)
     - 
     \rho\left( 
             \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                     \{ \ccalG \}
      \right)
\right\Vert
\end{multline}

xxxxxxxxxxxxxxxxxxxxxxxx


\begin{multline}
\left\Vert 
    \rho(\boldsymbol{a})
    -
    \rho\left( 
          \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                 \left(
                      \widehat{\ccalG}
                 \right)
         \right)
    -
    \boldsymbol{\xi} \{  \boldsymbol{p}_{\boldsymbol{a},\epsilon} \}
\right\Vert
\leq
\left\Vert 
   \rho(\boldsymbol{a})
    -
        \rho\left( 
             \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                     \{ \ccalG \}
        \right)
\right\Vert 
\\
+
\left\Vert 
    \rho\left( 
          \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                 \left(
                      \widehat{\ccalG}
                 \right)
         \right)
     - 
     \rho\left( 
             \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                     \{ \ccalG \}
      \right)
\right\Vert          
    +
    \left\Vert
         \boldsymbol{\xi} \{  \boldsymbol{p}_{\boldsymbol{a},\epsilon} \}
    \right\Vert
\end{multline}

xxxxxxxxxxxxxxxxxxxxxxx


\begin{multline}
\left\Vert 
    \rho(\boldsymbol{a})
    -
    \rho\left( 
          \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                 \left(
                      \widehat{\ccalG}
                 \right)
         \right)
    -
    \boldsymbol{\xi} \{  \boldsymbol{p}_{\boldsymbol{a},\epsilon} \}
\right\Vert
\leq
\left\Vert 
   \boldsymbol{a}
    -
   \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                     \{ \ccalG \}
\right\Vert 
\\
+
\left\Vert 
          \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                 \left(
                      \widehat{\ccalG}
                 \right)
     - 
          \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                     \{ \ccalG \}
\right\Vert          
    +
    \left\Vert
         \boldsymbol{\xi} \{  \boldsymbol{p}_{\boldsymbol{a},\epsilon} \}
    \right\Vert
\end{multline}


xxxxxxxxxxxxxxxxxxxxxxx


\begin{multline}
\left\Vert 
    \rho(\boldsymbol{a})
    -
    \rho\left( 
          \boldsymbol{p}_{\boldsymbol{a},\epsilon}
                 \left(
                      \widehat{\ccalG}
                 \right)
         \right)
    -
    \boldsymbol{\xi} \{  \boldsymbol{p}_{\boldsymbol{a},\epsilon} \}
\right\Vert
\leq
\epsilon 
\\
+
\left\Vert 
\bbD_{\boldsymbol{p}_{\boldsymbol{a},\epsilon}}(\ccalG)
\right\Vert          
\Vert \ccalG - \widehat{\ccalG} \Vert
    +
\vert 
  \ccalG
\vert
^{
\deg\left(
          \boldsymbol{p}_{\boldsymbol{a},\epsilon}
    \right)
    }\Delta
\end{multline}


xxxxxxxxxxxxxxxxxxxxxxx






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% SECTION %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Spectral Analysis}

Signal spectrum has been studied extensively in traditional signal processing. The latter are signal representations in the frequency domain, and are often used for property analysis, content compression, noise removal, and planning among others. We extend this concept to Lie signal processing by leveraging the representation theory of the Lie algebra. To be more precise, we start by introducing some basic operations between representations as follows.
%the homomorphism between representations as follows.
%
\begin{definition}[Homomorphism of representations]\label{def:homomorphismRepresentation}
	Let $(\ccalM_1, \rho_1)$ and $(\ccalM_2, \rho_2)$ be two representations of $U(\mathfrak{g})$ for a Lie algebra $\mathfrak{g}$. We say that a linear map $\phi: \ccalM_1 \to \ccalM_2$ is a homomorphism of representations if 
	%
	%
	%
	\begin{align}\label{eq:conditionHomomoRepresentation}
	\phi(\rho_1(g) v) = \rho_2(g) \phi(v),~\forall~v \in \ccalM_1,~g \in U(\mathfrak
	{g}). 
	\end{align}
	%
	%
	%
	If $\phi$ is also an isomorphism of vector spaces, then we say $\phi$ is an isomorphism of representations. 
\end{definition} 
%
\begin{definition}[Direct sum of representations]\label{def:directSumRepresentation}
	Let $(\ccalM_1, \rho_1)$ and $(\ccalM_2, \rho_2)$ be two representations of a Lie algebra $\mathfrak{g}$. The direct sum of $(\ccalM_1, \rho_1)$ and $(\ccalM_2, \rho_2)$ is defined as $(\ccalM_1 \oplus \ccalM_2, \rho)$ such that
	\begin{align}
	\rho(g)(v_1 \oplus v_2) = (\rho_1(g) v_1) \oplus (\rho_2(g)v_2)
	\end{align}
	for all $g \in \mathfrak{g},~v_1 \in \ccalM_1$ and $v_2 \in \ccalM_2$.
\end{definition}
\noindent Note that a homomorphism of representations is a homomorphism of vector spaces, while a homomorphism of vector spaces is not necessarily a homomorphism of representations since the condition \eqref{eq:conditionHomomoRepresentation} may not be satisfied. For the direct sum of representations, it provides a standard way for the representation decomposition. Specifically, the representation $(\ccalM, \rho) = (\ccalM_1 \oplus \ccalM_2, \rho)$ can be decomposed into two representations $(\ccalM_1, \rho_1)$ and $(\ccalM_2, \rho_2)$ with the operation of direct sum.

With these preliminaries in place, we introduce the indecomposable representation in the following definition.
%
\begin{definition}\label{def:indecomposableRepresentation}
	A nonzero representation $(\ccalM,\rho)$ of a Lie algebra $\mathfrak{g}$ is indecomposable if it is not isomorphic to a direct sum of two nonzero representations.
\end{definition}
%
\noindent The indecomposable representation provides the minimum unit of information that can be extracted from Lie signals defined on the vector space $\ccalM$ by Lie filters equipped with algebra structure $\mathfrak{g}$. The following theorem then establishes the decomposition of any finite dimensional representations.
%
\begin{theorem}\label{thm:decompositionRepresentation}
	Any finite dimensional representation of a Lie algebra can be decomposed into a finite direct sum of indecomposable representations, and the decomposition is unique up to the order of the summands and up to isomorphism.
\end{theorem} 
%
\noindent Theorem \ref{thm:decompositionRepresentation} states that there exists a unique decomposition for any finite dimensional representation. The uniqueness is subject to isomorphism and index ordering. That is, if the direct sum of indecomposable representations $\{(\ccalM_i, \rho_i)\}_{i=1}^m$ and $\{(\ccalV_j, \gamma_j)\}_{j=1}^v$ are isomorphic to each other $(\oplus_{i=1}^m \ccalM_i, \rho) \cong (\oplus_{j=1}^v \ccalV_i, \gamma)$, then $m = v$ and there exists a permutation $\pi$ of indices such that $(\ccalM_i, \rho_i) \cong (\ccalM_{\pi(j)}, \gamma_{\pi(j)})$. While guaranteeing the unique decomposition with respect to indecomposable representations, the vector space $\ccalM_i$ of the indecomposable representation are not necessarily invariant under its operators $\rho_i(g)$ for all $g \in \mathfrak{g}$. To overcome this issue, we consider the concept of irreducible representations in the following.
%
\begin{definition}
	Let $\mathfrak{g}$ be a Lie algebra and $(\ccalM, \rho)$ be a representation of $\mathfrak{g}$. Then, a representation $(\ccalU, \rho)$ of $\mathfrak{g}$ is a subrepresentation of $(\ccalM, \rho)$ if $\ccalU \subset \ccalM$ is invariant under all operations $\rho(g)$ for all $g \in \mathfrak{g}$, i.e., $\rho(g) u \in \ccalU$ for all $u \in \ccalU$ and $g \in \mathfrak{g}$. A representation $(\ccalM, \rho)$ with $\ccalM \ne 0$ is irreducible if the only subrepresentations of $(\ccalM, \rho)$ are $(0, \rho)$ and $(\ccalM, \rho)$.
\end{definition}
%
The irreducibility accounts for the invariance of the homomorphism $\rho$ during the representation decomposition. The class of irreducible representations of an algebra $\mathfrak{g}$ is denoted by $\text{Irr}{\mathfrak{g}}$. We follow to define a representation is completely reducible if it allows a decomposition with respect to irreducible subrepresentations.
%
\begin{definition}
	Let $\mathfrak{g}$ be a Lie algebra. A representation $(\ccalM, \rho)$ of $\mathfrak{g}$ is completely reducible if $(\ccalM, \rho)=\oplus_{i=1}^I (\ccalM_i, \rho_i)$ such that each subrepresentation $(\ccalM_i, \rho_i)$ is irreducible. The length of $(\ccalM,\rho)$ is defined as $I$.
\end{definition}
%
\noindent It is worth noting that irreducible subrepresentations are indecomposable, while indecomposable subrepresentations are not necessarily irreducible. We proceed to introducing some concepts that are relevant to the completely reducible representation decomposition.

For any representation $(\ccalM, \rho)$ and irreducible representation $(\ccalU,\rho_\ccalU) \in \text{Irr}(\mathfrak{g})$, denote by $\text{soc}\{\ccalM\}$ the direct sum of all irreducible subrepresentations of $(\ccalM, \rho)$ and $\ccalM(\ccalU)$ the direct sum of all irreducible subrepresentation of $(\ccalM,\rho)$ that are isomorphic to $(\ccalU,\rho_\ccalU)$. The former $\text{soc}\{\ccalM\}$ is completely reducible by definition, while the latter $\ccalM(\ccalU)$ is referred to as the $\ccalU$-homogeneous component of $(\ccalM, \rho)$. Moreover, denote by $m(\ccalM,\ccalU)$ the length of the direct sum in $\ccalM(\ccalU)$, referred to as the multiplicity of $(\ccalU,\rho_\ccalU)$ in $(\ccalM, \rho)$. The connection between $\text{soc}\{\ccalM\}$ and $\ccalM(\ccalU)$ is given by the following proposition.
%
\begin{proposition}\label{prop:relationSocHomo}
	Consider a representation $(\ccalM,\rho)$ of a Lie algebra $\mathfrak{g}$. Then, it holds that
	\begin{align}
	\text{soc}\{\ccalM\} = \oplus_{\ccalU \in \text{Irr}\{\mathfrak{g}\}} \ccalM(\ccalU).
	\end{align}
\end{proposition}
%
\noindent By leveraging the fact that homogeneous components $\ccalM(\ccalU)$ are direct sum of irreducible subrepresentations, we have
\begin{align}
\text{soc}\{\ccalM\} \cong \oplus_{\ccalU \in \text{Irr}\{\mathfrak{g}\}} \ccalU^{\oplus m(\ccalM,\ccalU)}.
\end{align}
The above discussion indicates that $\ccalM$ is completely reducible if and only if $\ccalM = \text{soc}\{\ccalM\}$, and its decomposition can be represented by the direct sum of homogeneous components $\ccalM(\ccalU)$ for all $\ccalU \in \text{Irr}\{\mathfrak{g}\}$. This establishes the theoretical foundation for the definition of Fourier decomposition in Lie signal processing. We formally define the latter in the following.
%
\begin{definition}[Fourier Decomposition]\label{def:FourierDecomposition}
	Consider the Lie signal processing model $(G, \ccalM, \mathfrak{g})$. There exists a Fourier decomposition of $(\ccalM,\rho)$ if
	\begin{align}
	\text{soc}\{\ccalM\} \cong \oplus_{(\ccalU_i,\rho_i) \in \text{Irr}\{\mathfrak{g}\}} \ccalU^{\oplus m(\ccalM,\ccalU_i)}.
	\end{align}
	where each $(\ccalU_i,\rho_i)$ is a irreducible subrepresentation of $(\ccalM,\rho)$. Then, for any Lie signal $\bbx \in \ccalM$, the Fourier decomposition of $\bbx$ is defined as the projection
	\begin{align}\label{eq:FourierDecomposition}
	\ccalM &\to \oplus_{(\ccalU_i,\rho_i) \in \text{Irr}\{\mathfrak{g}\}} \ccalU^{\oplus m(\ccalM,\ccalU_i)} \\
	\bbx &\to \hat{\bbx} \nonumber
	\end{align}
	where $\hat{\bbx}$ is the Fourier transformation of $\bbx$. The projection of $\hat{\bbx}$ in each $\ccalU_i$ are the Fourier components represented by $\hat{\bbx}(i)$.
\end{definition}
%
\noindent The Fourier decomposition in \eqref{eq:FourierDecomposition} contains two direct sums, where the external one is dedicated to non isomorphic subrepresentations and the internal one is dedicated to isomorphic subrepresentations. In this context, the direct sum of non isomorphic subrepresentations denotes the sum on the frequencies of the representation while the direct sum of isomorphic subrepresentations denotes the sum on components corresponding to the same frequency. 



%%-------------------------------
%%--------- THEOREM -------------
%%-------------------------------

\begin{theorem}(corollary 2.3.12 in~\cite{repthysmbook})
	Let $\ccalA$ be a commutative algebra. Then every
	irreducible finite dimensional representation $(\ccalM,\rho)$ of $\ccalA$ is 1-dimensional.
\end{theorem}



==> v24/theoretical_results.tex <==
\red{\section{Stability  Analysis ?}}

